Fingering instability in spreading epithelial monolayers: roles of cell polarisation, substrate friction and contractile stresses

Collective cell migration plays a crucial role in many developmental processes that underlie morphogenesis, wound healing, or cancer progression. In such coordinated behaviours, cells are organised in coherent structures and actively migrate to serve different biological purposes. In some contexts, namely during epithelial wound healing, it is well known that a migrating free-edge monolayer develops finger-like instabilities, yet the onset is still under debate. Here, by means of theory and numerical simulations, we shed light on the main mechanisms driving the instability process, analysing the linear and nonlinear dynamics of a continuum compressible polar fluid. In particular, we assess the role of cell polarisation, substrate friction, and contractile stresses. Linear theory shows that it is crucial to analyse the perturbation transient dynamics, since we unravel a plethora of crossovers between different exponential growth rates during the linear regime. Numerical simulations suggest that cell-substrate friction could be the mechanism responsible for the formation of complex finger-like structures at the edge, since it triggers secondary fingering instabilities and tip-splitting phenomena. Finally, we obtain a critical contractile stress that depends on cell-substrate friction and the initial-to-nematic length ratio, characterising an active wetting-dewetting transition. In the dewetting scenario, the monolayer retracts and becomes stable without developing finger-like structures.

==> aux.tex <==
We first consider a limit case with neither $\Lambda,\alpha,\beta\rightarrow 0$. In addition, the epithelial monolayer is polarized only in the boundary in which polarity modulus decays from $p = 1$ at the monolayer edge to $p = 0$ at the center. 
First, we write down the equations of the model in Cartesian coordinates considering a rectangular configuration typical of {\em in vitro} experiments.
The equations for the polarization field yields,
\begin{subequations}
\begin{gather}
(\partial^2_x +\partial^2_y)p_x = 0,\\
(\partial^2_x +\partial^2_y)p_y = 0
\end{gather}
\end{subequations}
and respectively, the equations for the velocity field reads
\begin{subequations}
\begin{gather}
(\partial^2_x +\partial^2_y)u_x + \partial_x(\partial_x u_x +\partial_y u_x) + p_x= 0, \\
(\partial^2_x +\partial^2_y)u_y + \partial_y(\partial_x u_y +\partial_y u_y)+p_y= 0
\end{gather}
\end{subequations}
We will assume that the base state of the system~\eqref{eq:pol}--\eqref{eq:mom} with $\lambda,\alpha,\beta\rightarrow 0$ is the flat-front solution, $y = L^0(t)$, whose expression for the polarization field $\boldm{p}^{0} = (0,p_y^0(y))$ and for velocity field $\boldm{u} = (0,u_y^0(y))$ are respectively
\begin{subequations}
\begin{gather}
p_y^0(y;t) = \frac{y}{ L^0(t)}, \\
u_y^0(y;t) = \frac{y L_0(t)}{4}\left(1-\frac{y^2}{3 L_0(t)^2} \right)
\end{gather}
\end{subequations}
To address the stability of the active fluid layer we linearize the base flow and then analyze the growth of the perturbations. The expression~\eqref{eq:normalmode} is introduced into~\eqref{eq:pol}, which yields the following normal-mode polarisation equations at leading order
\begin{subequations}
\begin{gather}
(\partial_x^2-k^2)p_x^1=0, \label{eq:p_1} \\
(\partial_x^2-k^2)p_y^1=0,
\end{gather}
\end{subequations}
to be solved with the following boundary conditions
\begin{subequations}
\begin{gather}
p_y^1 = \partial_y p_x^1 = 0\quad \text{at} \quad y = 0, \label{eq:nm_p_symmetry} \\
p_y^1 +\partial_y p_y^0 L^1 = 0, \quad p_x^1 +ik L^1 = 0 \quad \text{at} \quad y = L^0(t), \label{eq:nm_p_normal_tang} 
\end{gather}
\end{subequations}
Solving~\eqref{eq:p_1}--\eqref{eq:nm_p_normal_tang} yields
\begin{subequations}
\begin{gather}\label{eq:p1x_p1y}
p_x^1 = \frac{-i k L_1}{\text{cosh}(k L_0)}\text{cosh}(k y), \\
p_y^1 = \frac{-L_1}{L_0\, \text{sinh}(kL_0)}  \text{sinh}(k y).
\end{gather}
\end{subequations}
To obtain the normal-mode velocity field $(u_x^1,u_y^1)$, equation~\eqref{eq:normalmode} is introduced into the corresponding leading-order momentum equations~\eqref{eq:mom}
\begin{subequations}
\begin{gather}
(2\partial_{y}^2-k^2)u_y^ 1+ ik\partial_y u_x^ 1 + p_y^1=0, \label{eq:nm_u} \\
(\partial_{y}^2-2k^2)u_x^1+ ik\partial_y u_y^ 1+p_x^1 = 0,
\end{gather}
\end{subequations}
with associated boundary conditions
\begin{subequations}
\begin{gather}
u_y^1 = \partial_y u_x^1 = 0 \quad \text{at} \quad y = 0,\\
2 \partial_y u_y^1  + 2 \partial_y^2 u_y^0L_1=0 \quad y = L^0(t), \label{eq:nm_u_normal} \\
\partial_y u_x^1 + ik u_y^1 = 0  \quad \text{at} \quad y = L^0(t), \label{eq:nm_u_tangential}
\end{gather}
\end{subequations}
where we have assumed that $Ca \to \infty$. The system~\eqref{eq:nm_u}--\eqref{eq:nm_u_tangential} has been solved with Mathematica, and for conciseness $u_x^1$ and $u_y^1$ are not shown herein. Finally, the kinematic-condition~\eqref{eq:kinematic} at leading order yields
\begin{equation}
\frac{\text{d} L^1}{\text{d} t} = \partial_y u_y^0 \, L^1+u_y^1 \quad \text{at} \quad y = L^0(t). \label{eq:L1_eq}
\end{equation}
Since $u_y^1$ is proportional to $L^1$, we can define $u_y^1 = \hat{u}_y^1 L^1 $, and thus
the time-dependent growth rate reads
\begin{equation}
\omega(k,t) = \hat{u}_y^1(L_0),
\end{equation}
%and
%\begin{equation}\quad L^1(t) = \frac{-3 k L_0 - 4 k^3 L_0^3 - 5 \text{sinh}(2 k L_0) + k L_0 (9 \text{cosh}(2 k L_0) + 4 k L_0 \text{coth}(k L0) + 2 k L_0 \text{tanh}(k L_0)}{(8 k^2 L_0 (2 k L_0 + \text{sinh}(2 k L_0)))}.
%\end{equation}
